SecDDR: Enabling Low-Cost Secure Memories by Protecting the DDR Interface

The security goals of cloud providers and users include memory confidentiality and integrity, which requires implementing Replay-Attack protection (RAP). RAP can be achieved using integrity trees or mutually authenticated channels. Integrity trees incur significant performance overheads and are impractical for protecting large memories. Mutually authenticated channels have been proposed only for packetized memory interfaces that address only a very small niche domain and require fundamental changes to memory system architecture. We propose SecDDR, a low-cost RAP that targets direct-attached memories, like DDRx. SecDDR avoids memory-side data authentication, and thus, only adds a small amount of logic to memory components and does not change the underlying DDR protocol, making it practical for widespread adoption. In contrast to prior mutual authentication proposals, which require trusting the entire memory module, SecDDR targets untrusted modules by placing its limited security logic on the DRAM die (or package) of the ECC chip. Our evaluation shows that SecDDR performs within 1% of an encryption-only memory without RAP and that SecDDR provides 18.8% and 7.8% average performance improvements (up to 190.4% and 24.8%) relative to a 64-ary integrity tree and an authenticated channel, respectively.

==> text/old_abstract.tex <==
\begin{abstract}

The security goals of cloud providers and users include memory confidentiality and integrity, which requires implementing Replay-Attack protection (RAP). RAP can be achieved using integrity trees or mutually authenticated channels.  Integrity trees incur significant performance overheads and are impractical for protecting large memories. Mutually authenticated channels have been proposed only for packetized memory interfaces that address only a very small niche domain and require fundamental changes to memory system architecture. We develop low-cost RAP that targets direct-attached memory, like DDRx, which is therefore practical for the commodity market.

{\em Sentry} is a low-cost RAP framework based on the observation that practical Replay-Attacks modify the data while in motion, either on the bus or on the memory module. Sentry safeguards the bus against Replay-Attacks by encrypting the per-line MAC, ensuring that the MAC is temporally unique during the bus transfer and cannot be replayed. We develop Sentry for both trusted and untrusted memory modules and discuss associated trade-offs. 
%Although prior work has studied similar methods to create a replay-protected channel between the processor and the main memory, these proposals are mainly designed for the packetized protocols of the 3D-stacked memories, and adopting them requires fundamental changes to the design of a modern DDR memory module}. 
Sentry avoids memory-side MAC verification, and thus, only adds a small amount of logic (encryption units) to memory components and does not \makeblue{fundamentally} change the underlying DDR protocol, making it practical for widespread adoption. Our evaluation shows that Sentry performs within 3\% of an encryption-only memory without RAP and that Sentry provides 4.4\% and 6.1\% average performance improvements (up to 36.5\% and 14.4\%) relative to a 64-ary integrity tree and an authenticated channel, respectively.

\end{abstract}

==> text/security_discussion.tex <==
\section{Security Discussion}\label{sec:security-discussion}
\vspace{0.05 in}
\noindent{\bf Trusted DIMM \& On-DIMM Replay Attacks.}
\vspace{0.01 in}
In the threat model with a trusted DIMM,  Similarly to intercepting the bus, the on-DIMM trojan can intercept the on-DIMM traffic to replay the data. Note that the trojan must be relatively complex as it has to track, store, and precisely replay the 72-byte tuple for a specific address -- 80 bytes of information (72 tuple and 8 bytes of address). 

\ignore{
\vspace{0.05 in}
\noindent{\bf 3) Compatibility with Other Modes of Encryption.}
\vspace{0.01 in}
Recently introduced Intel TME~\cite{inteltme} and AMD SEV~\cite{amdsev} can encrypt the entire memory address space. These products use AES-XTS mode of encryption without relying on encryption counters. While this reduces the storage and memory bandwidth overhead of the memory encryption, lack of encryption counters makes implementing the state-of-the-art integrity trees impossible as they have to be built on the counters~\cite{yan2006improving}. One can use hash-based Merkle Trees, however, this incurs significant performance overhead (31.5\%) and compact and high-arity tree optimizations~\cite{saileshwar2018morphable, taassori2018vault} are hard to apply (higher arity reduces the hash length, increasing the collision probability). \papername{} can co-exist with the low-cost encryption in TME/SEV with negligible performance overhead (Section~\ref{sec:encryption-mode-sensitivity}).
}

\ignore{
%\subsection{Protecting Encryption-Counters in \papername{}}\label{sec:enc-count-protection}
In \papername{}, we do not distinguish between the data and the encryption counter lines. Encryption counters are also integrity-protected in a similar manner, using per-line MACs, as shown in Figure~\ref{fig:counter-line_protection}. Similar to the data lines, the processor will detect an attack that has occurred, but it cannot differentiate between different attack scenarios.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth]{graphs/counter_line_protection.pdf}
    \caption{Encryption counter protection in \papername{}.}
    \label{fig:counter-line_protection}
    \vspace*{-4mm}
\end{figure}
}
